Power Foam: Unifying Real-Time Differentiable Ray Tracing and Rasterization

We introduce a differentiable 3D representation that unifies the ray tracing capabilities of foam-based ray tracing with the efficiency of modern rasterization pipelines. While prior foam representations enable constant-time ray traversal through an explicit volumetric partition of space, their potentially unbounded cells hinder efficient tile-based rasterization. We address this limitation by generalizing Voronoi foams to bounded power diagrams with controllable cell extents, enabling spatially bounded primitives without requiring expensive Delaunay triangulations during training. We further introduce an oriented surface formulation that explicitly models interfaces between interior and exterior regions, and decouple geometry from appearance by embedding differentiable texture directly on these surfaces. Together, these contributions yield a representation that preserves state-of-the-art ray tracing efficiency while achieving rasterization performance competitive with current generation 3DGS, providing a practical path toward unified real-time differentiable rendering.

==> fig/method/item.tex <==
\begin{figure*}[t]
    \centering
    \begin{overpic}[width=0.24\linewidth]{fig/method/voronoi_diagram.png}
    \end{overpic}
    \begin{overpic}[width=0.24\linewidth]{fig/method/power_diagram.png}
    \end{overpic}
    \begin{overpic}[width=0.24\linewidth]{fig/method/localized_power_diagram.png}
    \end{overpic}
    \begin{overpic}[width=0.24\linewidth]{fig/method/dipoles.png}
    \end{overpic}
    \caption{
    {\bf Localized power diagram -- }
    }
    \label{fig:method}
\end{figure*}
